DiffusionFake: Enhancing Generalization in Deepfake Detection via Guided Stable Diffusion

The rapid progress of Deepfake technology has made face swapping highly realistic, raising concerns about the malicious use of fabricated facial content. Existing methods often struggle to generalize to unseen domains due to the diverse nature of facial manipulations. In this paper, we revisit the generation process and identify a universal principle: Deepfake images inherently contain information from both source and target identities, while genuine faces maintain a consistent identity. Building upon this insight, we introduce DiffusionFake, a novel plug-and-play framework that reverses the generative process of face forgeries to enhance the generalization of detection models. DiffusionFake achieves this by injecting the features extracted by the detection model into a frozen pre-trained Stable Diffusion model, compelling it to reconstruct the corresponding target and source images. This guided reconstruction process constrains the detection network to capture the source and target related features to facilitate the reconstruction, thereby learning rich and disentangled representations that are more resilient to unseen forgeries. Extensive experiments demonstrate that DiffusionFake significantly improves cross-domain generalization of various detector architectures without introducing additional parameters during inference. Our Codes are available in https://github.com/skJack/DiffusionFake.git.

==> sec/0_abstract.tex <==
\begin{abstract}


The rapid progress of Deepfake technology has made face swapping highly realistic, raising concerns about the malicious use of fabricated facial content. Existing methods often struggle to generalize to unseen domains due to the diverse nature of facial manipulations. In this paper, we revisit the generation process and identify a universal principle: Deepfake images inherently contain information from both source and target identities, while genuine faces maintain a consistent identity.
Building upon this insight, we introduce DiffusionFake, a novel plug-and-play framework that reverses the generative process of face forgeries to enhance the generalization of detection models. DiffusionFake achieves this by injecting the features extracted by the detection model into a frozen pre-trained Stable Diffusion model, compelling it to reconstruct the corresponding target and source images. This guided reconstruction process constrains the detection network to capture the source and target related features to facilitate the reconstruction, thereby learning rich and disentangled representations that are more resilient to unseen forgeries.
Extensive experiments demonstrate that DiffusionFake significantly improves cross-domain generalization of various detector architectures without introducing additional parameters during inference. Our Codes are available in \href{https://github.com/skJack/DiffusionFake.git}{https://github.com/skJack/DiffusionFake.git}.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}

The rapid progress in AI-generated content (AIGC) has led to the emergence of highly sophisticated forged face content, making it increasingly challenging for humans to distinguish between genuine and forged faces~\cite{rossler2019faceforensics++,zi2020wilddeepfake,dolhansky2020deepfake,chen2024diffusionface}. Face swapping, also known as \textit{Deepfakes}, is one of the most well-known techniques for generating forged facial images. It replaces the face of a target individual with that of a source person to create a seamless and realistic composite image~\cite{tolosana2020deepfakes}. The widespread proliferation of Deepfakes content on social media platforms has raised significant security concerns, including the spread of disinformation, fraud, and impersonation. As a result, developing effective and generalizable face forgery detection methods to counter these malicious attacks has become a critical challenge in the field of computer vision.

% The growing diversity of facial forgery techniques has spurred interest in the general face forgery detection task~\cite{sun2021domain}, which aims to develop models that detect forgeries from unseen domains. Previous approaches primarily utilize two strategies: forgery simulation and framework engineering~\cite{sun2023towards}. Forgery simulation, exemplified by methods like Face X-Ray\cite{li2020face} and SBI~\cite{shiohara2022detecting}, augments data by simulating blending artifacts, while SLADD~\cite{chen2022self} and VLFFD~\cite{sun2023towards} focus on more detailed forgery traces. Conversely, framework engineering enhances generalization through specialized designs, such as DCL~\cite{sun2021dual} using contrastive learning to differentiate features, and MAT~\cite{zhao2021multi} and SIA~\cite{sun2022information} applying attention mechanisms to capture subtle discrepancies. RECCE~\cite{cao2022end} employs reconstruction learning to distinguish between forged and genuine samples effectively.

The growing diversity of facial forgery techniques has spurred interest in the general face forgery detection task~\cite{sun2021domain}, which aims to develop models that detect forgeries from unseen domains. Previous approaches primarily utilize two strategies: forgery simulation and framework engineering~\cite{sun2023towards}. Forgery simulation augments data by simulating blending artifacts, as exemplified by methods like Face X-Ray\cite{li2020face} and SBI~\cite{shiohara2022detecting}. Other methods, such as SLADD~\cite{chen2022self} and VLFFD~\cite{sun2023towards}, focus on more detailed forgery traces. On the other hand, framework engineering enhances generalization through specialized designs. For instance, DCL~\cite{sun2021dual} uses contrastive learning to differentiate features, while MAT~\cite{zhao2021multi} and SIA~\cite{sun2022information} apply attention mechanisms to capture subtle discrepancies. RECCE~\cite{cao2022end} employs reconstruction learning to effectively distinguish between forged and genuine samples.

% In this paper, we aim to identify the universal features common to all Deepfake faces by revisiting the generation process of forged face images. As illustrated in Figure~\ref{fig:intro} (a), the process can be summarized at a high level as follows: a feature extractor module captures features from the source and target images, respectively. 
% These features are then combined through a generalized feature blending module to generate a new Deepfake image.
% While different forgery methods may vary in the feature extraction and blending modules, such as learning-based or graphics-based features eatractors, they consistently follow this generative paradigm.
% Through this analysis, we observe that Deepfake images inherently contain information from both source and target faces, while genuine images only contain consistent information.
In this paper, we aim to identify the universal features common to all Deepfake faces by revisiting the generation process of forged face images. As illustrated in Figure~\ref{fig:intro} (a), the process can be summarized at a high level as follows: a feature extractor module captures features from the source and target images, respectively. These features are then combined through a generalized feature blending module to generate a new Deepfake image. Although different forgery methods may vary in the feature extraction and blending modules, such as using learning-based or graphics-based feature extractors, they consistently follow this generative paradigm. Through this analysis, we observe that Deepfake images inherently contain information from both source and target faces, while genuine images only contain consistent information.

Building on this insight, we pose the question: \textit{Could we invert the generative process to extract and utilize these hybrid features for more effective detection?} To tackle the challenges associated with the loss of information during the forgery process, we leverage a state-of-the-art generative model, Stable Diffusion, to supplement this missing information. Our proposed framework, dubbed DiffusionFake, incorporates a plug-and-play training module that utilizes the reverse engineering of generative processes and disentangles source and target features through image restoration, as diagrammed in Figure~\ref{fig:intro} (b).


% Thus, we raise the following question: \textit{Could the detection process reverse the generation process and capture features related to the source and target images?} The resulting features will exhibit strong generalization properties.
% However, the inherent loss of information during the forgery process complicates the reconstruction of the original images from these incomplete features.
% To address this challenge, we leverage a powerful pre-trained generative model, Stable Diffusion, to augment such missing information. 
% Specifically, we propose the DiffusionFake, a plug-and-play training framework that can guide the detection module mine generalized forgery traces by reversing the generation process and disentangling the source and target features through image restoration.

which is diagrammed in Figure~\ref{fig:intro} (b). The process starts with the extraction and filtering of image features into source-related and target-related characteristics via the Feature Extractor and Feature Filter module. These features are then input into the Guide Module, which integrates them into the Stable Diffusion network for a latent diffusion training process aimed at reconstructing the respective source and target images. As genuine images represent the same individual, this process ensures that the features are reflective of the original identities.
Additionally, considering the varying levels of forgery detail across different images, we employ a Guided Weight Learning Module to adaptively determine the contribution of each sample to the pre-trained model during reconstruction.

In the testing phase, the system utilizes only the Feature Extractor and Discrimination Module to ascertain authenticity, enhancing generalization across various backbone architectures without the need for additional parameters. This streamlined approach not only simplifies implementation but also improves the robustness and adaptability of our detection framework.

The main contributions of our work can be summarized as follows:

\begin{itemize}
    \item We analyze forged face images from a generative perspective and propose a framework that exploits this reverse generation process to bolster the generalization capabilities of face forgery detectors.
    \item We introduce the DiffusionFake framework, incorporating a guided module with Stable Diffusion for image reconstruction, thereby enhancing the discriminative network's ability to identify generalizable features.

    \item Our extensive experimental validations demonstrate that the DiffusionFake framework significantly improves generalization capabilities across various architectures without necessitating additional inference parameters.
\end{itemize}

\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{fig/intro2.pdf}
    \end{center}
       \caption{Pipeline of the proposed lifelong face forgery detection (LFFD) setting.
       }
    \label{fig:intro}
\end{figure*}




% The amount and type of information from each source may vary depending on the specific forgery method employed. For instance, the NeuralTextures method results in relatively minor modifications, where the mouth movements and noise patterns in the forged face originate from the source face, while other regions are derived from the target face.
% For instance, in the learning-based Deepfake method, the facial expressions and certain attributes are inherited from the target, while the overall identity is derived from the source. Conversely, CG-based methods like NeuralTextures source the identity and expressions from the target, with only lip movements coming from the source, and blending limited to the mouth region.


% Based on the above observations, we hypothesize that if the detection process can reverse the generation process and capture features related to both the source and target images, the resulting features will exhibit strong generalization properties. 


% The growing variety of forged face generation techniques has led to increased interest in the \textit{general face forgery detection} task~\cite{sun2021domain}, which focuses on developing detection models from unseen domains and forgery types.
% Previous methods enhance generalization performance primarily through two approaches: \textit{forgery simulation} and \textit{framework engineering}~\cite{sun2023towards}.
% Forgery simulation methods focus on augmenting forged data by simulating specific forgery traces. For instance, Face X-Ray~\cite{li2020face} and SBI~\cite{shiohara2022detecting} enhance generalization by modeling blending artifacts, while SLADD~\cite{chen2022self} and VLFFD~\cite{sun2023towards} simulate more fine-grained forgery traces by blending different forged regions.
% On the other hand, framework engineering methods improve the generalization through special designs of learning frameworks. For example, DCL~\cite{sun2021dual} adopts a contrastive learning framework to increase the divergence between features, while MAT~\cite{zhao2021multi} and SIA~\cite{sun2022information} leverage attention mechanisms to enhance the capture of subtle features. RECCE~\cite{cao2022end} utilizes reconstruction learning to model authentic samples, thus enhancing the differentiation between unseen forged samples and genuine ones.

% Previous approaches have sought to enhance generalization performance from different perspectives. Methods such as LTW~\cite{sun2021domain}, DCL~\cite{sun2021dual}, MAT~\cite{zhao2021multi}, and CFM~\cite{luo2023beyond} focus on extracting more generalizable features to improve cross-domain performance. Other techniques, including Face X-ray~\cite{li2020face}, SLADD~\cite{chen2022self}, and SBI~\cite{shiohara2022detecting}, aim to simulate diverse forgery patterns and artifacts during training to better prepare the model for unseen forgeries. Additionally, UCF~\cite{yan2023ucf} tackles the generalization issue by decoupling the features learned by the detector to reduce overfitting to specific forgery methods. 

==> sec/1_intro_new.tex <==
\section{Introduction}

The rapid progress in AI-generated content (AIGC) has led to the emergence of highly sophisticated forged face content, making it increasingly challenging for humans to distinguish between genuine and forged faces~\cite{rossler2019faceforensics++,zi2020wilddeepfake,dolhansky2020deepfake,chen2024diffusionface}. Face swapping, also known as \textit{Deepfakes}, is one of the most well-known techniques for generating forged facial images. It replaces the face of a target individual with that of a source person to create a seamless and realistic composite image~\cite{tolosana2020deepfakes}. The widespread proliferation of Deepfakes content on social media platforms has raised significant security concerns, including the spread of disinformation, fraud, and impersonation. As a result, developing effective and generalizable face forgery detection methods to counter these malicious attacks has become a critical challenge in the field of computer vision.


The growing diversity of facial forgery techniques has spurred interest in the general face forgery detection task~\cite{sun2021domain,song2022adaptive,luo2023beyond}, which aims to develop models that detect forgeries from unseen domains. 
Previous approaches primarily utilize forgery simulation~\cite{li2020face,shiohara2022detecting,chen2022self,sun2023towards} to augment data by simulating various forgery traces, or framework engineering to enhance generalization through specialized designs like contrastive learning, attention mechanisms, and reconstruction learning~\cite{sun2021dual,zhao2021multi,sun2022information,cao2022end,gu2022hierarchical}. However, their generalization capabilities remain limited due to the reliance on simulating specific forgery artifacts or designing specialized architectures tailored to certain manipulation techniques.

In this paper, we aim to identify the universal features common to all Deepfake faces by revisiting the generative process underlying forged face images. As depicted in Figure~\ref{fig:intro} (a), this process can be distilled into two key steps: (1) a feature extractor module captures salient features from both the source and target images; (2) these features are seamlessly fused through a generalized feature blending module to synthesize a novel Deepfake image. While the specific implementation of feature extraction and fusion may vary across different forgery methods, ranging from learning-based to graphics-based approaches, they all adhere to this fundamental generative paradigm.

Through this analysis, we uncover a crucial insight: {Deepfake images inherently amalgamate information from both source and target faces, whereas genuine images maintain a consistent identity throughout}. This amalgamated information can manifest as low-level artifacts, such as injection noise patterns and spectral discrepancies, or as high-level attributes, including facial expressions and mouth movements, depending on the specific forgery method employed.

Building upon this insight, we raise a question: 
{Can we invert the generative process to extract and leverage the amalgamated source and target features, thereby enhancing the generalization capability of existing forgery detectors?}

To answer this question, we introduce {DiffusionFake}, a novel plug-and-play framework that harnesses the power of Stable Diffusion to guide the forgery detector in learning disentangled source and target features inherent in Deepfakes. The core idea behind DiffusionFake is to inject the features extracted by the detector into a frozen pre-trained Stable Diffusion model, compelling the detector to capture the amalgamated source and target information by optimizing the features to reconstruct the corresponding source and target images.

\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{fig/intro.pdf}
    \end{center}
    \vspace{-1em}
       \caption{Pipeline of the generation process of Deepfake (a) and our proposed DiffusionFake (b).
       }\vspace{-1em}
    \label{fig:intro}
\end{figure*}

As illustrated in Figure~\ref{fig:intro} (b), DiffusionFake is a plug-and-play framework that can be seamlessly integrated into existing forgery detectors. The features extracted by the encoder are first passed through the Target and Source Transformation modules, which filter and weight the features to obtain target and source-related representations. These features are then injected into the Stable Diffusion model using a Guide Module, leveraging its pre-trained knowledge to reconstruct the corresponding source and target images and optimize the feature representation. 

During inference, only the encoder and classification modules are used, ensuring no additional parameters or computational overhead. 
By compelling the detector to learn more discriminative and generalized features, DiffusionFake enhances its ability to handle unseen forgeries without compromising efficiency. For example, 
when integrated with EfficientNet-B4, DiffusionFake improves AUC scores on unseen Celeb-DF dataset by around 10\%, demonstrating its effectiveness in enhancing the generalization capability of existing detectors.

The main contributions of our work can be summarized as follows:
\vspace{-1em}
\begin{itemize}
    % [leftmargin=1em]
    % \setlength{\itemsep}{-0.0em}
    \item We analyze Deepfake images from a generative perspective and propose a framework that leverages the reverse generation process to enhance the generalization capabilities of face forgery detectors.
    \item We introduce the DiffusionFake framework, a plug-and-play model that integrates a frozen pre-trained Stable Diffusion network to guide the forgery detector in learning disentangled source and target features inherent in Deepfakes, further enhancing the generalization.
    \item Extensive experimental validations demonstrate that the DiffusionFake framework significantly improves generalization capabilities across various architectures without introducing additional inference parameters.
\end{itemize}


==> sec/2_related.tex <==
\section{Related Work}
\subsection{General Face Forgery Detection}
General face forgery detection aims to improve the performance of forgery detectors on unseen domains and become one of the most critical issues in this field.
Previous work to enhance generalization can be broadly divided into two categories: forgery simulation and framework engineering. The former utilizes data augmentation methods to simulate certain forgery traces, such as blending artifacts~\cite{guillaro2023trufor,li2020face,shiohara2022detecting}, Inconsistency between internal and external faces~\cite{zhao2021learning}, subtle jitter and blur traces~\cite{larue2023seeable}, and fine-grained facial disharmony~\cite{chen2022self,sun2023towards}. The latter improves network architectures or training procedures to help capture more generalized traces.
Such methods approach the problem from different angles. Some employ attention mechanisms to enhance the capture of forgery traces~\cite{zhao2021multi,sun2022information,xu2023tall,shao2023detecting}, while others improve generalization by jointly modeling frequency and spatial domains~\cite{qian2020thinking,li2021frequency,luo2021generalizing,liu2021spatial}. Reconstruction-based methods enhance discriminability against unseen domain forgeries via modeling genuine faces~\cite{chen2021magdr,cao2022end,shi2023real}. Additionally, some approaches use implicit identity as a clue to improve the generalization of Deepfake faces~\cite{huang2023implicit,dong2023implicit} and some explore the local and global relationships of unseen forgeries\cite{chen2021local,bai2023aunet,wang2023dynamic,guillaro2023trufor,dong2022explaining,luo2021capsule}. Furthermore, decoupling methods\cite{liang2022exploring,shao2022detecting,guo2023controllable,le2023quality}, such as ICT~\cite{dong2022protecting} and UCF~\cite{yan2023ucf}, aim to enhance generalization by disentangling different facial information. Our DiffusionFake method addresses this by reversing the forgery process and leveraging pre-trained generative models to complete missing information, enhancing the capture of source-related and target-related features.



\subsection{Diffusion Model}

Diffusion models have emerged as a powerful framework for image generation and manipulation. The seminal work on Denoising Diffusion Probabilistic Models (DDPM)~\cite{ho2020denoising} introduced a novel approach to learn the data distribution by iteratively denoising a Gaussian noise signal. This process allows for high-quality image generation but requires a large number of sampling steps. To address this issue, the Denoising Diffusion Implicit Models (DDIM)~\cite{song2020denoising} proposed a deterministic sampling process that significantly accelerates the generation process while maintaining image quality. Building upon these advancements, the Latent Diffusion Model (LDM)~\cite{rombach2022high} combines the strengths of Variational Autoencoders (VAEs)~\cite{kingma2013auto} and diffusion models. 
By applying the diffusion process in the latent space learned by a VAE, LDM substantially reduces the computational cost and memory requirements during training. 
This innovative architecture has given rise to powerful AIGC pre-trained generative models, such as Stable Diffusion~\footnote{https://stability.ai/news/stable-diffusion-public-release}, which enable high-quality image generation and manipulation with unprecedented efficiency.
Recent developments in controllable diffusion models have further expanded their applicability. ControlNet~\cite{zhang2023adding}introduces a mechanism to guide the image generation process by conditioning the diffusion model on additional control signals, such as segmentation masks or edge maps. Inspired by ControlNet, our DiffusionFake leverages a guide module to inject the source and target-related features into Stable Diffusion to reconstruct the corresponding images.



==> sec/3_method.tex <==
\section{Methodology}
% Figure~\ref{fig:main} illustrates the detailed framework of our proposed DiffusionFake method. First, a generic encoder is employed to extract features from the input face image. Simultaneously, we aim to capture features related to both the source and target faces present in the forged image. Two structurally identical feature filters are used to extract the corresponding source and target features, which are subsequently fed into the guide module. This module guides a fixed-parameter Stable Diffusion model to reconstruct the target and source images, encouraging the encoder to learn more generalizable features. Furthermore, considering that the amount of source and target information varies among different attack types, we introduce a weight module to adaptively control the dependency on the guided information during the diffusion process.


Figure~\ref{fig:main} illustrates the detailed framework of our proposed DiffusionFake method, which aims to enhance the generalization capability of forgery detectors by guiding the learning of amalgamated source and target features through a frozen pre-trained Stable Diffusion model. Specifically, the features extracted by the encoder are first filtered and weighted by the Feature Filter and Weight Modules to obtain source and target-related representations. These features are then injected into a frozen pre-trained Stable Diffusion model via the Guide Module, which reconstructs the corresponding source and target images, compelling the encoder to learn rich and discriminative features. 



\subsection{Preliminaries}
\textbf{Diffusion Process.} Denoising Diffusion Probabilistic Models (DDPMs)~\cite{ho2020denoising} are latent variable models that learn to generate data by reversing a gradual noising process. The forward diffusion process gradually adds Gaussian noise to the data $x_0$ according to a variance schedule $\beta_1, \dots, \beta_T$, producing a sequence of noisy samples $x_1, \dots, x_T$. The forward process can be described as:
\begin{equation}
q(x_t|x_{t-1}) = \mathcal{N}(x_t; \sqrt{1-\beta_t}x_{t-1}, \beta_t\mathbf{I})
\end{equation}
The reverse denoising process learns to generate samples from the data distribution by starting with a Gaussian noise sample $x_T$ and iteratively denoising it using a learned denoising function $\epsilon_\theta$. The reverse process is defined as:
\begin{equation}
p_\theta(x_{t-1}|x_t) = \mathcal{N}(x_{t-1}; \mu_\theta(x_t, t), \sigma_t^2\mathbf{I}),
\end{equation}
% where
\begin{equation}
\mu_\theta(x_t, t) = \frac{1}{\sqrt{\alpha_t}} \left( x_t - \frac{1-\alpha_t}{\sqrt{1-\bar{\alpha}t}} \epsilon_\theta(x_t, t) \right),
\end{equation}

$\alpha_t = 1 - \beta_t$, $\bar{\alpha}_t = \prod_{s=1}^t \alpha_s$, and $\sigma_t^2 = \frac{1-\bar{\alpha}_{t-1}}{1-\bar{\alpha}_t}\beta_t$.
The training objective is to minimize the weighted sum of the denoising error at each step:
\begin{equation}
L = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,1), t \sim [1, T]} \left[ || \epsilon - \epsilon_\theta(x_t, t) ||_2^2 \right]
\end{equation}

\textbf{Stable Diffusion.}
The Stable Diffusion Model is a powerful pre-trained model with impressive generative capabilities, able to synthesize various types of images, including different types of human faces.
Built upon the DDPM framework, the Stable Diffusion models employs a Latent Diffusion Model (LDM)~\cite{rombach2022high} to reduce resource consumption. LDM applies the diffusion process in a learned latent space instead of pixel space, which is obtained by training an autoencoder. 
The training objective is:
\begin{equation}
L = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,1), t \sim [1, T]} \left[ || \epsilon - \epsilon_\theta(z_t, t) ||_2^2 \right],
\end{equation}
where $z_t$ is the latent representation encoded by the VAE encoder. This strategic application of latent space modeling not only enhances efficiency but also preserves the high quality of generated images.

\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{fig/main2.pdf}
    \end{center}
    \vspace{-1em}
       \caption{The details of the DiffusionFake method. The blue arrow represents the target branch, the red arrow represents the source branch, the {\footnotesize\color{blue} \SnowflakeChevronBold}~represents the parameter frozen and does not participate in training, and the {\footnotesize\color{red} \faFire} represents the trainable module.
       }
    \label{fig:main}
\end{figure*}

\subsection{Feature Transformation}

% \textbf{Notation}: 
Given an input image $x$ and its corresponding label $y$, where $y=0$ represents a real face and $y=1$ represents a forged face, let $x_s$ and $x_t$ denote the corresponding source and target images from the training dataset, respectively. For real faces, $x_s$ and $x_t$ are identical to $x$. Let $E$ be the encoder, and the extracted features be $f = E(x)$.
To transform the extracted feature $f$ 
into components that can guide the Stable Diffusion process, we first 
introduce two key modules: the \textit{Feature Filter Module} and the \textit{Weight Module}.

\textbf{Feature Filter Module.} The Feature Filter Module $F$ is to extract source-related and target-related features from the encoded features $f$. To achieve this, we employ two filter networks, $F_s$ and $F_t$, to obtain the source-related feature $f_s = F_s(f)$ and target-related feature $f_t = F_t(f)$, respectively.

As shown in Figure~\ref{fig:main}, the Feature Filter Module combines convolutional layers and attention mechanisms. The features first pass through a convolutional layer to transform the channels. Then channel-wise~\cite{hu2018squeeze} and spatial-wise attention~\cite{woo2018cbam} are applied to adaptively weight and filter the features. These attention mechanisms help to emphasize the most relevant features while suppressing less informative ones, leading to more discriminative representations.

Subsequently, a Multi-Head Attention mechanism~\cite{vaswani2017attention} is then applied to perform cross-attention between the original features (query) and the attention-filtered features (key and value). This operation captures long-range dependencies and enhances the receptive field, enabling more effective feature refinement. 
Finally, to ensure compatibility with the encoder of the Stable Diffusion model, we apply upsampling and pooling operations to align the feature dimensions.

% Subsequently, a Multi-Head Attention mechanism is used to perform cross-attention, where the original features serve as the query, and the attention-filtered features serve as the key and value. This cross-attention operation enables the model to capture long-range dependencies and enhance the receptive field of the filtered features, allowing for more effective feature refinement and adaptation. Finally, to match the feature dimensions with the encoder of the Stable Diffusion model, we employ upsampling and pooling operations for feature alignment.

\textbf{Weight Module.} The Weight Module $W$ addresses the varying levels of source and target information embedded in different types of forged images. For example, Deepfakes may evenly blend source and target features, while expression-driven methods like NeuralTextures may predominantly feature target image information with minimal source information confined to specific regions like mouth movements. Uniformly feeding these into the guide module would be suboptimal.

To mitigate this, we use two separate weight modules, $W_s$ and $W_t$, to estimate the information content for source and target features. Each weight module start with a pooling layer, following five MLP layers, and a sigmoid function finally outputs the weight. We train these modules using the similarity scores between the input image and its respective source and target images as ground truth.

Specifically, we encode $x$, $x_t$, and $x_s$ using the pre-trained VAE-Encoder from Stable Diffusion to obtain latent representations $z$, $z_t$, and $z_s$. Such a well-pretrained model can effectively capture and quantify the differences between images, providing a reliable basis for measuring the similarity between the input image and its corresponding source and target images.
The similarity scores between $z$ and $z_t$, and between $z$ and $z_s$, are computed and used to train the weight modules with mean squared error (MSE) loss as follows:
\begin{equation}
\mathcal{L}_{ws} = \left||W_s(f) - \text{sim}(z, z_s)\right||_2^2
\end{equation}
\begin{equation}
\mathcal{L}_{wt} = \left||W_t(f) - \text{sim}(z, z_t)\right||_2^2
\end{equation}
where $\text{sim}(a, b) = \frac{a \cdot b}{|a| |b|}$ denotes the cosine similarity between vectors $a$ and $b$.

By dynamically adjusting the influence of source and target features during the diffusion process, the Weight Module ensures optimal guidance for the Stable Diffusion model, thereby enhancing the encoder's ability to extract generalized features suitable for detecting a wide range of forgeries.

\subsection{Guide Module}
% The Guide Module is designed to inject the source-related and target-related features into the frozen pre-trained Stable Diffusion model to guide the reconstruction of the source and target images. The architecture of the Guide Module is illustrated in Figure~\ref{fig:main}.


The Guide Module is designed to inject the source-related and target-related features into the frozen pre-trained Stable Diffusion model to guide the reconstruction of the source and target images. As illustrated in Figure~\ref{fig:main}, the Guide Module employs trainable copy and zero convolution layers for feature injection, inspired by ControlNet~\cite{zhang2023adding}.


Let $U_E(\cdot)$ and $U_D(\cdot)$ denote the neural block of the encoder and decoder in the U-Net $\epsilon_\theta$ network of the Stable Diffusion model, respectively. The Guide Module first creates a trainable copy of $U_E(\cdot)$, denoted as $U_E^{'}(\cdot)$. The source-related feature $f_s$ and target-related feature $f_t$ are then independently fed into $U_E^{'}(;)$. The resulting features are combined with the corresponding features from the locked model's decoder $U_D(;)$ using zero convolution layers $Z(\cdot)$, which are $1\times1$ convolutional layers with weights and biases initialized to zeros. This initialization minimizes the impact on the pre-trained model at the beginning of training, stabilizing the training process~\cite{zhang2023adding}. The final output of the Guide Module can be summarized as:

% Inspired by ControlNet~\cite{zhang2023adding}, we employ trainable copy and zero convolution layers for feature injection. Let $U_E(\cdot)$ and $U_D(\cdot)$ denote the neural block of the encoder and decoder in the U-Net $\epsilon_\theta$ network of the Stable Diffusion model, respectively. The Guide Module first creates a trainable copy of $U_E(\cdot)$, denoted as $U_E^{'}(\cdot)$.

% The source-related feature $f_s$ and target-related feature $f_t$ are then independently fed into $U_E^{'}(;)$. The resulting features are combined with the corresponding features from the locked model's decoder $U_D(;)$ using zero convolution layers $Z(\cdot)$. These layers are simple $1\times1$ convolutional layers with both weights and biases initialized to zeros, which has been shown to minimize the impact on the pre-trained model at the beginning of training, thereby stabilizing the training process~\cite{zhang2023adding}. The final output of the Guide Module can be summarized as:

\begin{equation}
fs^{'} = U_D(U_E(z_s)) + Z(U_E^{'}(f_s)) \times W_s(f)
\end{equation}
\begin{equation}
ft^{'} = U_D(U_E(z_t)) + Z(U_E^{'}(f_t)) \times W_t(f)
\end{equation}
where $z_s$ and $z_t$ are the latent representations of the source and target images, respectively, obtained from the pre-trained VAE-Encoder of Stable Diffusion, and $W_s(f)$ and $W_t(f)$ are the weights computed by the Weight Module.

Unlike ControlNet, which aims to control the generated results of the diffusion model, our objective is to optimize the features $f$ by fixing the output and encouraging the capture of more generalizable and disentangled features. By guiding the reconstruction of the source and target images using the respective features, the Guide Module facilitates the learning of rich and discriminative representations that enhance the performance of the forgery detector across various domains and attack types.

% Note that while ControlNet aims to control the generated results of the diffusion model, our objective is to optimize the features $f$ by fixing the output and encouraging the capture of more generalizable and disentangled features. By guiding the reconstruction of the source and target images using the respective features, the Guide Module facilitates the learning of rich and discriminative representations that enhance the performance of the forgery detector across various domains and attack types.

% During training, we follow a process similar to the LDM~\cite{rombach2022high}. We gradually execute the diffusion process, including the time step $t$, to guide the reconstruction of the source and target images. 

% At each time step $t$, the model learns to predict the noise $\epsilon$ that was added to the latent representation of the source or target image. The overall learning objective for the source and target diffusion models can be formulated as:
During training, we follow a process similar to the LDM~\cite{rombach2022high}, gradually executing the diffusion process, including the time step $t$, to guide the reconstruction of the source and target images. At each time step $t$, the model learns to predict the noise $\epsilon$ that was added to the latent representation of the source or target image. The overall learning objective for the source and target diffusion models can be formulated as:

\begin{equation}
L_s = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,1), t \sim [1, T]} \left[ || \epsilon - \epsilon_\theta(fs_{t}^{'}, t) ||_2^2 \right]
\end{equation}
\begin{equation}
L_t = \mathbb{E}_{\epsilon \sim \mathcal{N}(0,1), t \sim [1, T]} \left[ || \epsilon - \epsilon_\theta(ft_{t}^{'}, t) ||_2^2 \right]
\end{equation}
where ${fs}_{t}^{'}$ and $ft_{t}^{'}$ represent the features within the embedding of time step $t$. 

\subsection{Loss Function and Inference}
% For classification, 
We apply a simple binary classification head to the extracted feature $f$ to obtain the predicted label $y'$, which is calculated via typical cross-entropy loss as follows: 
% The cross-entropy loss is then calculated as follows:
\begin{equation}
L_{ce} = - \left[ y \log y' + (1 - y) \log (1 - y') \right] \label{eq:ce}
\end{equation}

Thus, the final loss function combines Eq.\ref{eq:ce} with the losses from our \textit{Weight module} and \textit{Gudie module}, which is defined as follows:
% diffusion process:
\begin{equation}
L = L_{ce} + \lambda_s L_s + \lambda_t L_t + L_{ws} + L_{wt}
\end{equation}
where $\lambda_s$ and $\lambda_t$ are hyperparameters that balance the contributions of the source and target diffusion losses, $L_s$ and $L_t$, respectively.

% Since the diffusion process ensures that the encoder network extracts generalized features, during inference, we only retain the Encoder and the classification head. 
\textbf{Inference.}
During inference, only the Encoder and the classification head are retained, as shown in the purple dotted box in Figure \ref{fig:main}. It is worth noting that DiffusionFake ensures the encoder network extracts generalized features only during training. Consequently, our DiffusionFake framework does not introduce any additional parameters during inference, thereby enhancing generalizability and reducing computational overhead.
% During inference, we only retain the Encoder and the classification head, as shown in the purple dotted box in the purple dotted box in Figure \ref{fig:main}.
% It's worth noting that the DiffusionFake ensures that the encoder network extracts generalized features, only during training. 
% This means that our DiffusionFake framework does not introduce any additional parameters during inference, thus enhancing generalizability and reducing computational overhead.



==> sec/4_experiment.tex <==
\section{Experiment}
\label{sec:experiment}
\subsection{Experimental Setting}
\textbf{Dataset.}
To evaluate the generalization ability of DiffusionFake, we conduct experiments on several challenging datasets:
(1) FaceForensics++ (FF++)~\cite{rossler2019faceforensics++}: This widely-used dataset contains 1,000 videos with four manipulation methods: DeepFakes, NeuralTextures, Face2Face, and FaceSwap. The pairwise real and forged data enable the generation of mixed forgery images. (2) Celeb-DF~\cite{li2019celeb}: A high-quality DeepFake dataset containing various scenarios.  (3) DeepFake Detection (DFD): This dataset comprises 363 real videos and 3,068 fake videos, primarily generated using the DeepFake method. (4) DFDC Preview (DFDC-P)~\cite{dolhansky2020deepfake}: A challenging dataset with 1,133 real videos and 4,080 fake videos, featuring various manipulation methods and backgrounds. (5) WildDeepfake~\cite{zi2020wilddeepfake}: A diverse dataset obtained from the internet, capturing a wide range of real-world scenarios. (6) DiffSwap~\cite{chen2024diffusionface}: A recently released dataset containing 30,000 high-quality face swaps generated using the diffusion-based DiffSwap method~\cite{zhao2023diffswap} on the MM-Celeb-A dataset. This dataset allows for evaluating cross-method generalization.

\textbf{Training details.}
DiffusionFake is a plug-and-play architecture that can be integrated with different backbone networks by simply adjusting the dimensions of the alignment layer in the Feature Filter module. During training, we utilize a pre-trained Stable Diffusion 1.5 model with frozen parameters. Input images are resized to 224$\times$224 pixels. We employ the Adam optimizer with a learning rate of 1e-5 and a batch size of 32. The model is trained for 20 epochs. The hyperparameters $\lambda_s$ and $\lambda_t$ are set to 0.7 and 1, respectively. We employ widely used data augmentations, such as HorizontalFlip, and CutOut. To ensure a fair comparison, we follow the data split strategy used in FaceForensics++~\cite{rossler2019faceforensics++}. The overall framework is implemented in Pytorch on one NVIDIA A-100 GPU.



% \input{table/table1}
\input{table/table1_new}
\subsection{Experimental Results}
We use AUC and EER to evaluate all the methods, including ours, both of them are widely used in deepfake detection.\footnote{More details about the evaluation metrics can be found in the appendix.}
We compare DiffusionFake with several state-of-the-art methods.

\textbf{Cross-dataset evaluation.} To validate the generalization capability of DiffusionFake, we first evaluate its performance on unseen datasets against recent state-of-the-art methods. Following previous settings, we train the models on the FF++ dataset and test them on several unseen domain datasets. The frame-level results are shown in Table~\ref{table:1}, where * denotes results obtained using official code with consistent training settings and data.

We evaluate its performance using two representative backbones: EfficientNet-B4 (En-B4) and ViT-B. We observe that incorporating DiffusionFake significantly improves the generalization ability of both architectures compared to their original classification backends. For En-B4, our method boosts performance on Celeb-DF by 11\% and achieves an average improvement of 6\%. Similarly, ViT-B sees a 6\% increase on DFDC and an average gain of 6\% when trained with DiffusionFake. Remarkably, \textbf{these enhancements are achieved without increasing the parameter count or computational overhead during inference}.
Compared to state-of-the-art methods, DiffusionFake outperforms disentanglement-based approaches like UCF and CAADM on Celeb-DF. Moreover, our method demonstrates substantial improvements on the latest diffusion-based face swapping dataset, DiffSwap, highlighting its effectiveness against the most recent forgery techniques. These results validate the ability of the guide module and Stable Diffusion network to encourage the encoder to learn more generalizable features by reconstructing source and target images. Due to space limitations, we provide the results of single-source and multi-source cross-manipulation evaluations in the appendix.


\subsection{Ablation Study}

\textbf{Ablation of components.}
% The proposed DiffusionFake consists of several key modules: 1) the pre-trained Stable Diffusion (SD) model, 2) the Feature Filter module, and 3) the Weight Module. Thus we conducted an ablation study to investigate the impact of these modules on our method.
% The results are shown in 
% Table~\ref{table:4}. Note that the model without SD refers to not loading the pre-trained weights of the SD model, while without Filter means directly feeding the encoder's output features $f$ into the guide module.
We conducted an ablation study to investigate the impact of the key modules in DiffusionFake: 1) the pre-trained Stable Diffusion (SD) model, 2) the Feature Filter module, and 3) the Weight Module. The results are shown in Table~\ref{table:ablation}, where without SD refers to not loading the pre-trained weights of the SD model, and without Filter means directly feeding the encoder's output features $f$ into the guide module.

We can observe that the pre-trained Stable Diffusion model is crucial for the DiffusionFake framework. Without the pre-trained weights, the network struggles to reconstruct the source and target images due to information loss, hindering the training process. Furthermore Both the Feature Filter and Weight modules play significant roles, and removing either of them leads to a performance decline. Specifically, eliminating the Filter module results in a 5\% AUC drop, as the filtering component allows the reconstruction to focus on relevant information without interference from redundant features. On the other hand, the absence of the Weight module causes a 3\% performance decrease, as this module assesses the amount of source and target information contained in the image, providing a prior for the generative network to determine the importance of guided information during the reconstruction process.

\textbf{Ablation of backbones.}
As our method can be flexibly embedded into different backbones by adjusting the alignment of the Feature Filter, we conduct an ablation study on various backbone architectures to demonstrate the versatility of DiffusionFake. We experiment with traditional ResNet-34, lightweight EfficientNet-B0, and the ViT-based ViT-Small. The results in Table~\ref{table:backbone} show that integrating our method into these backbones significantly improves generalization performance. For instance, applying DiffusionFake to the lightweight EfficientNet-B0 increases the generalization accuracy on Celeb-DF from 71.75\% to 76.31\%, surpassing the original EfficientNet-B4 (73.51\%). This evidence suggests that our method can effectively drive different encoders to extract more generalizable features.


\input{table/ablation}

\begin{figure*}[t!]
    \vspace{-1em}
    \begin{center}
    \includegraphics[width=0.95\textwidth]{fig/vis_rec3.pdf}
    \end{center}
    \vspace{-1em}
       \caption{Reconstruction results of DiffusionFake for training (A) and unseen (B) samples. For unseen samples, the model is provided with three sets of initial Gaussian noise, differing only in the injected guide information. The numbers below represent the Euclidean distance between the corresponding source and target features.
       }\vspace{-1em}
    \label{fig:vis_rec}
\end{figure*}

\subsection{Analysis and Visualizations}


\textbf{Visualizations of reverse results.}
Figure \ref{fig:vis_rec} showcases the reconstruction results for both training and unseen samples using DiffusionFake. For training samples (Figure \ref{fig:vis_rec} A), DiffusionFake effectively reconstructs the target image, despite the source image being slightly blurry due to information loss, capturing the basic characteristics of the ground truth. 
In order to compare the reconstruction effect more intuitively, we use the RECCE method to directly reconstruct the source and target images of the fake image. It can be seen that the reconstruction effect is very poor. In contrast, the reconstruction effect of our method is better due to the help of the pre-trained SD model.
For unseen samples (Figure \ref{fig:vis_rec} B), fake images with mixed features result in significant differences between reconstructed target and source images, while real images exhibit smaller differences. The Euclidean distances at the bottom quantify these differences, indicating larger differences in fake images compared to real ones.
% supporting the conclusions from Figure \ref{fig:vis_hist}.

% Figure \ref{fig:vis_rec} visualizes the reconstruction results of both training and unseen samples using DiffusionFake.
% For training samples, Figure \ref{fig:vis_rec} (A) demonstrates that DiffusionFake effectively reconstructs the target image. Although the source image appears slightly blurry due to significant information loss, it still captures the basic characteristics of the ground truth. In contrast, Figure \ref{fig:vis_rec} (B) illustrates that for unseen samples, the fake image containing mixed features leads to substantial differences between the reconstructed target and source images, while real images display smaller differences. To quantify these differences, the Euclidean distances of the corresponding features are provided at the bottom of the figure. These distances reveal that the differences in fake images are considerably larger than those in real images, which aligns with the conclusions derived from Figure \ref{fig:vis_hist}.

\textbf{Analysis of feature divergence. }
DiffusionFake utilizes two Feature Filter modules to separate source-related and target-related features, expecting significant divergence between $f_s$ and $f_t$ for forged images and minimal differences for genuine faces. To validate this, we visualize the Euclidean distance distribution between these features across various datasets, including FFpp, Celeb-DF, Wild-Deepfake, and DiffSwap, as shown in Figure \ref{fig:vis_hist}. The plots clearly distinguish real from fake samples: real samples have small feature distances, mostly within 0.05, whereas fake samples show larger distances due to mixed source and target information. These observations strongly support that DiffusionFake effectively disentangles source and target information in the extracted features.







% DiffusionFake employs two Feature Filter modules to disentangle source-related and target-related features, anticipating a substantial divergence between $f_s$ and $f_t$ for forged images and minimal differences for genuine faces.
% To validate this hypothesis, we visualize the distribution of Euclidean distances between the two features across various datasets, including FFpp, Celeb-DF, Wild-Deepfake, and DiffSwap, as shown in Figure \ref{fig:vis_hist}. The plots reveal a clear distinction between real and fake samples. For real samples, the distances between the two features are relatively small, primarily concentrated within 0.05. In contrast, fake samples, which inherently contain information from both the source and target identities, exhibit larger distances between $f_s$ and $f_t$, reflecting the substantial differences in their feature representations.
% These observations provide strong evidence that our proposed DiffusionFake framework effectively disentangles the source and target information within the extracted features. 

\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=1.0\textwidth]{fig/vis_hist2.pdf}
    \end{center}
    \vspace{-1em}
       \caption{Histogram of feature divergence on FFpp, Celeb-DF, Wild-Deepfake, and DiffSwap.
       }
       
    \label{fig:vis_hist}
\end{figure*}
\textbf{Analysis of feature distribution.}
To demonstrate that DiffusionFake enhances the discriminative power and generalization ability of the extracted features, we visualize the t-SNE plots of the last layer features from two encoders: the original EfficientNet-B4 (En-B4) and En-B4 trained with DiffusionFake. The feature distributions are examined on two unseen datasets, Celeb-DF and Wild-Deepfake.
As illustrated in Figure \ref{fig:tsne}, the original En-B4 exhibits poor generalization on both datasets, with the real and fake features being nearly inseparable. In contrast, when trained with DiffusionFake, the encoder learns to capture the generalizable hybrid features present in forged images via the reverse process. Consequently, the real and fake features become more distinctly separated, forming clear decision boundaries on both unseen datasets. 


\begin{figure*}[t!]
    \begin{center}
    \includegraphics[width=0.95\textwidth]{fig/vis_tsne2.pdf}
    \end{center}
    \vspace{-1em}
       \caption{Feature distribution of En-b4 model and the En-b4 model trained with our DiffusionFace on two unseen datasets Celeb-DF and Wild-Deepfake via t-SNE. The red represents the real samples while the blue represents the fake ones.
       }
    \label{fig:tsne}
\end{figure*}





==> sec/5_conclusion.tex <==
\section{Conclusion}
In this paper, we introduce DiffusionFake, a novel framework that leverages the generative process of face forgery to enhance the generalization capabilities of detection models. DiffusionFake inverts this generative process to extract and utilize hybrid features from source and target identities for effective forgery detection. Extensive experiments demonstrate that DiffusionFake significantly improves the generalization performance of various detector architectures without increasing inference parameters. 
The proposed framework enables the learning of discriminative and generalizable features, enhancing the robustness of detectors against a wide range of unseen forgeries.

% \textbf{Limitation.}
% The framework requires paired source and target images for training, which may not always be feasible. We aim to integrate self-supervised methods to generate these images in the future.

==> table/table1.tex <==

% \begin{table*}[!h]
%     \renewcommand\arraystretch{1.1}
%     \centering
%     \resizebox{0.95\textwidth}{!}{
%     \begin{tabular}{l|cc|cccccccc}
%     % \begin{tabular}{|ccccccccccc|}
%     \hline
%     \multirow{2}*{Method} & \multicolumn{2}{c|}{\textit{FF++}}&\multicolumn{2}{c}{DFD} & \multicolumn{2}{c}{DFDC-P} & \multicolumn{2}{c}{Wild Deepfake} &\multicolumn{2}{c}{Celeb-DF}\\
%     % \cline{2-11}
%     \cmidrule{2-3}
%     \cmidrule{3-11}

    

%     & AUC& EER &AUC& EER& AUC& EER& AUC& EER& AUC& EER\\
%     \hline
%     Xception~\cite{chollet2017xception}& 99.09&3.77 &87.86& 21.04& 69.80& 35.41&66.17 &40.14 & 65.27& 38.77\\
%     % \hline
%     EN-b4~\cite{tan2019efficientnet}   &99.22 &3.36& 87.37      & 21.99      & 70.12       & 34.54      & 61.04           & 45.34           & 68.52         & 35.61        \\
%     % \hline
%     Face X-ray~\cite{tan2019efficientnet}& 87.40&-& 85.60&-& 70.00&      -      &       -          &         -        & 74.20          &       -       \\
%     % \hline
%     % MLDG          &98.99 &3.46    & 88.14      & 21.34      & 71.86       & 34.44      & 64.12           & 43.27           & 74.56         & 30.81        \\
%     % \hline
    
%     % \hline
%     F3-Net~\cite{qian2020thinking}          & 98.10& 3.58 & 86.10     & 26.17       &     72.88       &      33.38      & 67.71          &      40.17           & 71.21        &     34.03         \\
%     MAT~\cite{zhao2021multi} & 99.27&3.35& 87.58      & 21.73      & 67.34       & 38.31      & 70.15           & 36.53           & 70.65         & 35.83        \\
%     % \hline
%     GFF~\cite{luo2021generalizing}             & 98.36& 3.85 & 85.51      & 25.64      & 71.58       & 34.77      & 66.51           & 41.52            & 75.31         & 32.48        \\
%     % \hline
%     LTW~\cite{sun2021domain}            & 99.17& 3.32  & 88.56      & 20.57      & 74.58       & 33.81      & 67.12           & 39.22           & 77.14         & 29.34         \\
    
%     % \hline
%     LRL~\cite{chen2021local}    & \textbf{99.46}&\textbf{3.01}& 89.24      & 20.32      & 76.53       & 32.41      & 68.76           & 37.50              & 78.26         & 29.67        \\
    
%     DCL~\cite{sun2021dual}              & 99.30&3.26& 91.66      & 16.63      & 76.71       & 31.97      & 71.14         & 36.17           & 82.30       & 26.53   \\
%     PCL+I2G~\cite{zhao2021learning}& 99.11&-& -      & -      & -       & -      & -         & -           & 81.80       & -   \\
%     SBI~\cite{shiohara2022detecting}    & 88.33&20.47&88.13&17.25&76.53&30.22&68.22&38.11&80.76&26.97 \\
%     UIA-ViT~\cite{zhuang2022uia} &-&-&94.68&-&75.80&-&-&-&82.41&- \\
%     RECCE~\cite{cao2022end} &99.32&3.38&89.91&19.95&75.88&32.41&67.93&39.82&70.50&35.34 \\
%     UCF~\cite{yan2023ucf} &97.05&-&80.74&-&75.94&-&-&-&75.27&- \\

%     % UIA-ViT   & 99.33&-&94.68&-&75.80&-&-&-&82.41&- \\
%     \hline

%     Ours              & 99.23&3.12& \textbf{94.79}      & \textbf{15.31}      & \textbf{84.74}       & \textbf{23.43}      & \textbf{83.55}           & \textbf{24.40}           & \textbf{84.80}          & \textbf{22.73}       \\

%     % Ours+Enhance              & 99.10&3.23& \textbf{95.05}      & \textbf{15.22}      & \textbf{85.22}       & \textbf{22.94}      & \underline{81.94}           & \underline{27.64}           & \textbf{85.22}          & \textbf{22.54}       \\

    
%     \hline

%     \end{tabular}
%     }
%     \caption{\textbf{Frame-level} cross-database evaluation from FF++(HQ) to DFD, DFDC-P, Wild Deepfake and Celeb-DF in terms of AUC and EER. The FF++ belongs to the intra-domain results while others represent the unseen-domain.
%     }
%     \label{table:1}
%     \end{table*}




% \begin{table*}[!h]
%     \renewcommand\arraystretch{1.1}
%     \centering
%     \resizebox{0.95\textwidth}{!}{
%     \begin{tabular}{l|cccccccccc}
%     % \begin{tabular}{|ccccccccccc|}
%     \hline
%     \multirow{2}*{Method} & \multicolumn{2}{c}{\textit{DiffSwap}}&\multicolumn{2}{c}{DFD} & \multicolumn{2}{c}{DFDC-P} & \multicolumn{2}{c}{Wild Deepfake} &\multicolumn{2}{c}{Celeb-DF}\\
%     % \cline{2-11}
%     \cmidrule{2-3}
%     \cmidrule{3-11}

    

%     & AUC& EER &AUC& EER& AUC& EER& AUC& EER& AUC& EER\\
%     \hline
%     Xception~\cite{chollet2017xception}& 99.09&3.77 &87.86& 21.04& 69.80& 35.41&66.17 &40.14 & 65.27& 38.77\\
%     % \hline
%     EN-b4~\cite{tan2019efficientnet}   &99.22 &3.36& 87.37      & 21.99      & 70.12       & 34.54      & 61.04           & 45.34           & 68.52         & 35.61        \\
%     % \hline
%     Face X-ray~\cite{tan2019efficientnet}& 87.40&-& 85.60&-& 70.00&      -      &       -          &         -        & 74.20          &       -       \\
%     % \hline
%     % MLDG          &98.99 &3.46    & 88.14      & 21.34      & 71.86       & 34.44      & 64.12           & 43.27           & 74.56         & 30.81        \\
%     % \hline
    
%     % \hline
%     F3-Net~\cite{qian2020thinking}          & 98.10& 3.58 & 86.10     & 26.17       &     72.88       &      33.38      & 67.71          &      40.17           & 71.21        &     34.03         \\
%     MAT~\cite{zhao2021multi} & 99.27&3.35& 87.58      & 21.73      & 67.34       & 38.31      & 70.15           & 36.53           & 70.65         & 35.83        \\
%     % \hline
%     GFF~\cite{luo2021generalizing}             & 98.36& 3.85 & 85.51      & 25.64      & 71.58       & 34.77      & 66.51           & 41.52            & 75.31         & 32.48        \\
%     % \hline
%     LTW~\cite{sun2021domain}            & 99.17& 3.32  & 88.56      & 20.57      & 74.58       & 33.81      & 67.12           & 39.22           & 77.14         & 29.34         \\
    
%     % \hline
%     LRL~\cite{chen2021local}    & \textbf{99.46}&\textbf{3.01}& 89.24      & 20.32      & 76.53       & 32.41      & 68.76           & 37.50              & 78.26         & 29.67        \\
    
%     DCL~\cite{sun2021dual}              & 99.30&3.26& 91.66      & 16.63      & 76.71       & 31.97      & 71.14         & 36.17           & 82.30       & 26.53   \\
%     PCL+I2G~\cite{zhao2021learning}& 99.11&-& -      & -      & -       & -      & -         & -           & 81.80       & -   \\
%     SBI~\cite{shiohara2022detecting}    & 88.33&20.47&88.13&17.25&76.53&30.22&68.22&38.11&80.76&26.97 \\
%     UIA-ViT~\cite{zhuang2022uia} &-&-&94.68&-&75.80&-&-&-&82.41&- \\
%     RECCE~\cite{cao2022end} &99.32&3.38&89.91&19.95&75.88&32.41&67.93&39.82&70.50&35.34 \\
%     UCF~\cite{yan2023ucf} &97.05&-&80.74&-&75.94&-&-&-&75.27&- \\

%     % UIA-ViT   & 99.33&-&94.68&-&75.80&-&-&-&82.41&- \\
%     \hline

%     Ours              & 99.23&3.12& \textbf{94.79}      & \textbf{15.31}      & \textbf{84.74}       & \textbf{23.43}      & \textbf{83.55}           & \textbf{24.40}           & \textbf{84.80}          & \textbf{22.73}       \\

%     % Ours+Enhance              & 99.10&3.23& \textbf{95.05}      & \textbf{15.22}      & \textbf{85.22}       & \textbf{22.94}      & \underline{81.94}           & \underline{27.64}           & \textbf{85.22}          & \textbf{22.54}       \\

    
%     \hline

%     \end{tabular}
%     }
%     \caption{\textbf{Frame-level} cross-database evaluation from FF++(HQ) to DFD, DFDC-P, Wild Deepfake and Celeb-DF in terms of AUC and EER. The FF++ belongs to the intra-domain results while others represent the unseen-domain.
%     }
%     \label{table:1}
%     \end{table*}


\begin{table*}[!t]
    \renewcommand\arraystretch{1.1}
    \centering
    \caption{\textbf{Frame-level} cross-database evaluation from FF++(HQ) to Celeb-DF, DFD, DFDC-P, Wild Deepfake and DiffSwap in terms of AUC and EER. * represents the results reproduced using open-source code or model.  
}
    \label{table:1}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l|ccccccccccc}
    % \begin{tabular}{|ccccccccccc|}
    \hline
    \multirow{2}*{Method} & \multicolumn{2}{c}{Celeb-DF} & \multicolumn{2}{c}{DFD} & \multicolumn{2}{c}{DFDC-P} & \multicolumn{2}{c}{Wild Deepfake} & \multicolumn{2}{c}{DiffSwap}\\
    \cmidrule{2-11}
    & AUC & EER & AUC & EER & AUC & EER & AUC & EER & AUC & EER\\
    \hline
    Xception~\cite{chollet2017xception} & 65.27 & 38.77 & 87.86 & 21.04 & 69.80 & 35.41 & 66.17 & 40.14 & 74.25 & 32.04\\
    
    
    Face X-ray~\cite{tan2019efficientnet} & 74.20 & - & 85.60 & - & 70.00 & - & - & - & - & -\\
    F3-Net*~\cite{qian2020thinking} & 71.21 & 34.03 & 86.10 & 26.17 & 72.88 & 33.38 & 67.71 & 40.17 & 76.89 & 30.83\\
    MAT*~\cite{zhao2021multi} & 70.65 & 35.83 & 87.58 & 21.73 & 67.34 & 38.31 & 70.15 & 36.53 & 79.93 & 27.77\\
    GFF*~\cite{luo2021generalizing} & 75.31 & 32.48 & 85.51 & 25.64 & 71.58 & 34.77 & 66.51 & 41.52 & 78.38 & 28.15\\
    LTW~\cite{sun2021domain} & 77.14 & 29.34 & 88.56 & 20.57 & 74.58 & 33.81 & 67.12 & 39.22 & 77.95 & 29.01\\
    LRL~\cite{chen2021local} & 78.26 & 29.67 & 89.24 & 20.32 & 76.53 & 32.41 & 68.76 & 37.50 &- & -\\
    DCL~\cite{sun2021dual} & 82.30 & 26.53 & 91.66 & 16.63 & 76.71 & 31.97 & 71.14 & 36.17 & 80.21 & 27.37\\
    PCL+I2G~\cite{zhao2021learning} & 81.80 & - & - & - & - & - & - & - & - & -\\
    SBI*~\cite{shiohara2022detecting} & 80.76 & 26.97 & 88.13 & 17.25 & 76.53 & 30.22 & 68.22 & 38.11 & 75.20 & 31.49\\
    UIA-ViT~\cite{zhuang2022uia} & 82.41 & - & \textbf{94.68} & - & 75.80 & - & - & - & - & -\\
    RECCE*~\cite{cao2022end} & 70.50 & 35.34 & 89.91 & 19.95 & 75.88 & 32.41 & 67.93 & 39.82 & 77.59 & 29.38\\
    UCF~\cite{yan2023ucf} & 75.27 & - & 80.74 & - & 75.94 & - & - & - & - & -\\
    CADDM*~\cite{dong2023implicit} & 77.56 & 30.63 & 82.90 & 25.20 & 72.45 & 33.56 & 72.56 & 33.63 & 75.58 & 31.01\\
    
    EN-b4*~\cite{tan2019efficientnet} & 73.51 & 34.17 & 87.57 & 21.31 & 70.51 & 33.98 & 70.04 & 37.03 & 77.38 & 29.44\\
    VIT-B*~\cite{tan2019efficientnet} & 74.64 & 33.07 & 84.38 & 24.15 & 74.24 & 34.29 & 75.46 & 31.53 & 78.50 & 28.14\\
    \hline
    % En-b4+Ours & \textbf{83.17}$_{\uparrow{9.12}}$ & \textbf{24.59}$_{\uparrow{9.12}}$ & 91.71$_{\uparrow{9.12}}$ & \textbf{16.27}$_{\uparrow{9.12}}$ & \textbf{77.35}$_{\uparrow{9.12}}$ & \textbf{30.17}$_{\uparrow{9.12}}$ & \textbf{75.17}$_{\uparrow{9.12}}$ & \textbf{33.25}$_{\uparrow{9.12}}$ & \textbf{82.02}$_{\uparrow{9.12}}$ & \textbf{25.55}$_{\uparrow{9.12}}$\\
    
    En-b4+Ours & \textbf{83.17} & \textbf{24.59} & 91.71 & \textbf{16.27} & 77.35 & 30.17 & 75.17 & 33.25 & 82.02 & 25.55\\
    
    VIT-B+Ours & 80.46 & 27.51 & 90.36 &19.73 & \textbf{80.95} & \textbf{27.66} & \textbf{80.14} & \textbf{29.62} & \textbf{86.98} & \textbf{21.32}\\
    \hline
\end{tabular}
}

\end{table*}
